TL;DR Progress: Multi-faceted Literature Exploration in Text Summarization

This paper presents TL;DR Progress, a new tool for exploring the literature on neural text summarization. It organizes 514~papers based on a comprehensive annotation scheme for text summarization approaches and enables fine-grained, faceted search. Each paper was manually annotated to capture aspects such as evaluation metrics, quality dimensions, learning paradigms, challenges addressed, datasets, and document domains. In addition, a succinct indicative summary is provided for each paper, consisting of automatically extracted contextual factors, issues, and proposed solutions. The tool is available online at https://www.tldr-progress.de, a demo video at https://youtu.be/uCVRGFvXUj8

==> figure-indicative-summary-prompts.tex <==
\begin{figure}[ht]
\centering
\begin{tcolorbox}[colback=gray!10!,colframe=blue!45!black,title=\tt{\small Context Factors Prompt (GPT3.5)}]
\small
You are a helpful assistant that can read and analyze scientific papers. You are given the following paper: \{\emph{Introduction}\} \newline 
Answer the following three questions: (1) Why are the authors generating the summaries of the documents? (2) Who are they for? (3) How will they be used? You must not include the proposed approach by the authors for generating the summaries. 
\newline \newline 
You will output a list of the question-answer pairs where each question is prefixed by the token QUESTION: and each answer is prefixed by the ANSWER: token. Each pair is separated by two lines.
\end{tcolorbox}
\begin{tcolorbox}[colback=gray!10!,colframe=blue!45!black,title=\tt{\small Problems and Solutions Prompt (GPT3.5)}]
\small
You are a helpful assistant that can read and analyze scientific papers. You are given the following paper: \{\emph{Introduction}\} \newline \newline
Can you give me a list of the main problems tackled by the authors and their proposed solutions? In this list, each problem is described followed by a solution proposed by the authors. Each problem starts with the token PROBLEM and each solution starts with the token SOLUTION. \newline \newline 
Here is the list:
\end{tcolorbox}
\caption{Prompts for extracting contextual information from the introduction of a paper. This information is used to compose indicative summaries of papers. The specific instructions for controlling output format may not be required with newer models.}
\label{fig:indicative-summary-prompts}
\end{figure}

==> figure-terminology-extraction-prompts.tex <==
\begin{figure}[ht]
\centering
\begin{tcolorbox}[colback=gray!10!,colframe=brown!65!black,title=\tt{\small Glossary Prompt (GPT3.5)}]
\small
You are a scientist who can read and summarize scientific papers. You are given the following paper: \{\emph{Introduction}\}. Your task is to extract a list of key concepts along with correct definitions like a glossary of the paper. Follow the format [\emph{Concept}: \emph{Definition}].
\end{tcolorbox}
\begin{tcolorbox}[colback=gray!10!,colframe=brown!65!black,title=\tt{\small Acronyms Prompt (GPT3.5)}]
\small
You are a scientist who can read and summarize scientific papers. You are given the following paper: \{\emph{Introduction}\}. Your task is to extract a list of acronyms that the authors use along with correct expansions from the paper. 
\newline \newline
For example (1)~EDU: Elementary Discourse Unit, (2)~SEHY: Simple Yet Effective Hybrid Model, (3)~PLM: Pretrained Language Model. Exclude acronyms for which no expansion is explicitly provided by the authors. Follow the format [\emph{Acronym}: \emph{Expansion}].
\end{tcolorbox}
\caption{Prompts for automatic terminology acquisition from the introduction of a paper. We extract glossary as well as acronym-expansion pairs. For the latter, we provide examples of the expected output format.}
\label{fig:terminology-extraction-prompts}
\end{figure}
